End-to-End Application Cloning for Distributed Cloud Microservices with Ditto

We present Ditto, an automated framework for cloning end-to-end cloud applications, both monolithic and microservices, which captures I/O and network activity, as well as kernel operations, in addition to application logic. Ditto takes a hierarchical approach to application cloning, starting with capturing the dependency graph across distributed services, to recreating each tier's control/data flow, and finally generating system calls and assembly that mimics the individual applications. Ditto does not reveal the logic of the original application, facilitating publicly sharing clones of production services with hardware vendors, cloud providers, and the research community. We show that across a diverse set of single- and multi-tier applications, Ditto accurately captures their CPU and memory characteristics as well as their high-level performance metrics, is portable across platforms, and facilitates a wide range of system studies.

==> Discussion.tex <==
\section{Discussion}
% \label{sec:ditto-discussion}


\subsection{Suitable and Unsuitable Use Cases}
Ditto’s main contribution is cloning an end-to-end application across the system stack. This makes it more suitable for architecture-, OS-, application-, and cluster-level studies, including scalability, networking, threading, interference, and power management. It can also be used for certain microarchitecture studies, as we showed when changing memory hierarchies across platforms.

However, to enable fast, automated, and obfuscated cloning, our method abstracts away the original individual instructions and memory accesses. Thus, it is less accurate for microarchitecture studies that rely on exact application implementation rather than their statistical performance patterns. For instance, studying the memory access patterns to improve hardware prefetchers would not be a good fit for Ditto. There is a fundamental trade-off between the granularity at which information is captured in one subsystem, and the overall performance accuracy.

\subsection{Confidentiality}

Although Ditto cannot guarantee zero information leakage, as it may expose the RPC graph, and statistics of some hardware counters, many software companies do not consider these sensitive data. For example, Alibaba, has open-sourced their production RPC traces~\cite{alibaba_trace}, Facebook shared the kernel-level cycles breakdown of its production workloads~\cite{accelerometer}, and Google open-sourced their workload traces via DynamoRIO~\cite{48320}. Additionally, the application skeleton, while may reflect the original workflow to some extent, is chosen and adapted from the network and threading models that have been extensively studied and used~\cite{fan2015performance, utune, zhang2019impact}. As the actual logic, functionality and per-access memory patterns are concealed, inferring useful proprietary information would be very difficult.

For collaboration with hardware vendors, sharing the proprietary code under NDA is of course a more straightforward way, but most cloud providers would not share the binaries related to their core business regardless of NDA agreements. Other solutions like internal evaluation of prototypes can be time-consuming and inaccurate since the prototype is usually immature, and cloud providers need to adapt their workloads for each new prototype.

\subsection{Application Phases}

Previous studies observe execution phases in SPEC CPU benchmark applications ~\cite{hamerly2005simpoint,isci2005long}. To verify whether program phases exists in the evaluated cloud services, we collect time series of CPU metrics spanning 600 seconds, with sampling frequencies ranging from one second to ten seconds. We do not observe regular program phases with such sampling granularity. There may be program phases in the execution of individual requests, which range from tens of microseconds to tens of milliseconds. Nevertheless, they rarely manifest across requests, unless caused by load fluctuations, which Ditto captures. As the service processes hundreds of requests per second, the overall program phases are averaged across concurrent requests. 

\subsection{Multi-tenancy and Virtualization}
We demonstrate Ditto's accuracy in local, virtualized, and multi-tenant deployments in Sections~\ref{sec:ditto-validation} and~\ref{sec:ditto-evaluation_interference}. Although we do not directly model contention and hypervisor events, the behavior of synthetic and target applications under multi-tenancy and virtualization is similar. In Ditto, the synthetic application clones the interference sensitivity by matching the target application's resource usage patterns. The performance overhead of virtualization comes primarily from network and disk I/O, nested paging, VM scheduling, and OS interactions~\cite{7095802}. Cloning the network and thread models, system calls and memory accesses ensures that synthetic and original applications experience similar overheads. 


\subsection{Limitations and Future Work}
Ditto currently only supports C/C++ applications compiled for x86 ISA, as it relies on instrumentation tools designed for C/C++ and x86. However, Ditto does not depend on any language- or ISA-specific features, and can be easily adapted to other languages and ISAs. 

Cloning for specialized hardware, such as GPUs, FPGAs, and smartNICs is also gaining in importance. Due to their radically different ISAs and computing paradigms, we leave extending Ditto for them to future work. 

